FUNU: Boosting Machine Unlearning Efficiency by Filtering Unnecessary Unlearning

Machine unlearning is an emerging field that selectively removes specific data samples from a trained model. This capability is crucial for addressing privacy concerns, complying with data protection regulations, and correcting errors or biases introduced by certain data. Unlike traditional machine learning, where models are typically static once trained, machine unlearning facilitates dynamic updates that enable the model to ``forget'' information without requiring complete retraining from scratch. There are various machine unlearning methods, some of which are more time-efficient when data removal requests are fewer. To decrease the execution time of such machine unlearning methods, we aim to reduce the size of data removal requests based on the fundamental assumption that the removal of certain data would not result in a distinguishable retrained model. We first propose the concept of unnecessary unlearning, which indicates that the model would not alter noticeably after removing some data points. Subsequently, we review existing solutions that can be used to solve our problem. We highlight their limitations in adaptability to different unlearning scenarios and their reliance on manually selected parameters. We consequently put forward FUNU, a method to identify data points that lead to unnecessary unlearning. FUNU circumvents the limitations of existing solutions. The idea is to discover data points within the removal requests that have similar neighbors in the remaining dataset. We utilize a reference model to set parameters for finding neighbors, inspired from the area of model memorization. We provide a theoretical analysis of the privacy guarantee offered by FUNU and conduct extensive experiments to validate its efficacy.

==> PH1.tex <==
Our method PH1 aims to select a subset of unlearning dataset $D_u$ to form $D_u^+$ such that the samples in $D_u^+$ have similar neighbors in $D_r$. The contribution of these samples would be replaced by neighbors in $D_r$, rendering them less significant to the retrained model. Consequently, unlearning operations can bypass these samples.

In detail, PH1 has three steps, as illustrated in Figure \ref{fig:proceedure}. First, calculate the distance matrix based on features generated by the original trained model $M_o$. Second, use a reference model $M_{ref}$ to establish the similarity condition $Sim(x, D)$. If a sample $x$ and a dataset $D$ satisfy this condition, i.e. $Sim(x, D) = True$, then the sample $x$ would be considered to have sufficient similar neighbors in $D$. Third, we compare samples in $D_u$ with $D_r$ using the similarity condition established in the previous step and select $D_u^+$. 

\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/method-crop}
  \caption{The proceedure of PH1}
  \label{fig:proceedure}
\end{figure}

\subsection{Calculate distance matrix}
\label{sec:calculate_distance_matrix}

The distance matrix, denoted as $M^{d}$, is a matrix whose dimensions correspond to the size of the original dataset, i.e., $M^{d} \in \mathbb{R}^{N \times N}$, where $N = |D_o|$. Each cell of $M^{d}$ represents a distance between two samples, such that $M_{i,j}^{d} = sample\_distance(x_i, x_j)$, where $x_i,x_j \in D_o$. 

We now introduce the function above $sample\_distance$ in detail. We first use the original model $M_o$ to generate the feature representation of a given sample $x$. Specifically, we use the model output before the last fully connected layer as the feature representation of the given sample, denoted as $M_{f}(x)$. We use the features generated by models instead of the original input to measure similarity from the view of the model. Next, for each sample pair in $D_o$, we calculate their cosine distance to construct the distance matrix. Combining these two steps, we have $sample\_distance(x_i, x_j) = cos(M_f(x_i), M_f(x_j))$, which implements the distance matrix. It is important to note that the larger the cosine distance, the more similar the two samples are.

\subsection{Establish similarity condition}
\label{sec:establish_similarity_condition}

The similarity condition $Sim(x, D)$ determines whether a sample $x$ has a sufficient number of similarity neighbors in dataset $D$, such that the contribution of $x$ to a model trained on $D$ could be considered negligible.

We formulate the similarity condition as follows. $Sim_{\theta, \alpha}(x, D) = True$ if there are more than $\alpha$ samples $\{y_1,...,y_{\alpha*}\}, \alpha* \ge \alpha$, $y_i \in D$ that satisfies $sample\_distance(x, y_i) \ge \theta$. That is if there are enough samples in $D$ considered similar to $x$, $Sim_{\theta, \alpha}(x, D)$ will return true.

In the first step, we have already calculated the distance matrix, so the $sample\_distance(x, y)$ for each sample pair is known. The key problem in establishing the similarity condition is to determine the parameters, $\alpha$ and $\theta$. Instead of manually choosing parameters, we use a reference model to find similar samples first, and derive the statistics of those samples to set the parameters.

%In the first step, we have the distance between each sample pair in $D_o$. Next, we would solve this problem: Given a sample $x \in D_u$ and remained dataset $D_r$, to what similarity condition can we claim $x$ has enough similar neighbors in $D_r$ so that it can be removed from $D_u$? 

%We further specify the confition as follows. Given a sample $x \in D_u$, $D_x = {y | y \in D_r, dist(x, y)\ge \theta}$, if $|D_x| \ge \alpha$, then $x$ has sufficient similar neighbors in $D_r$ and thus can be removed from $D_u$. Our task is to decide the threshold $\theta$ and $\alpha$.  

Our reference model $M_{ref}$ is acquired as follows. We initialize a model that has the same structure as the original model and train it on $D_o$ for one epoch. The resulting model is designated as the reference model. This design is motivated by two key considerations.

First, regarding the effectiveness of this reference model in addressing our problem, since the reference model just iterates over the whole dataset for one epoch, it has seen each data sample only once. In this case, we infer the samples correctly predicted by $M_{ref}$ have sufficient similar neighbors in the entire dataset, enabling the model to make correct predictions. This inference is consistent with the findings in ~\cite{agarwal2022estimating, wei2024memorization}, which suggest that models tend to learn patterns at the early training stage. $M_{ref}$ is a model at an early stage of training (one epoch). The data samples being predicted correctly could be recognized as contributing to pattern learning, and thus hold common characteristics. Second, in view of efficiency, the reference model is straightforward to implement. It does not require additional datasets for training and only necessitates training for one epoch, thereby conserving computational resources and time.

Samples that can be correctly predicted by $D_o$ are considered similar within each class. We denote $D_c^{ref}$ as the samples in class $c$ that are correctly predicted by $M_{ref}$. Then we use the statistics of $D_i^{ref}$ across different classes to be our parameters for $Sim_{\theta, \alpha}$. Specifically, $$\theta_c = avg(sample\_distance(x_i, x_j)),  x_i, x_j \in D_c^{ref}$$ $$\theta = avg(\theta_c), \  c \in C $$ where $C$ is the set of classes. Within each class $c$, we count the average number $\alpha_c$ as $$\alpha_c = count(\{(x_i, x_j) | sample\_distance(x_i, x_j) \ge \theta \}), x_i, y_i \in D_c^{ref}$$ The final $\alpha$ is given by: $$\alpha = avg(\alpha_c), \ c \in C$$

\subsection{Filter removal requests}
\label{sec:filter_removal_requests}

We utilize the distance matrix $M^d$ and the parametized similar condition $Sim_{\theta, \alpha}(x, D)$ to filter samples in $D_u$ that have more than $\alpha$ similar neighbors, i.e., $D_u^+ = \{x|x\in D_u \ and \  Sim_{\theta, \alpha}(x, D_r) = True \}$. Specifically, we select a sub-matrix of $M^d$, which contains distances between samples in $D_u$ and $D_r$, and we perform filtering on this sub-matrix. The samples regarded as $D_u^+$ are removed from $D_u$. The remaining samples, denoted as $D_u^-$, are those that require unlearning.

It is noteworthy that this step has to be executed whenever data removal requests are received, as the remaining dataset $D_r$ changes each time. As demonstrated in our experiment (Section \ref{sec:time_cost}), this incurs additional time costs compared to alternative methods, but also increases its adaptivity to various unlearning scenarios.

==> alternative_methods_v0_1015.tex <==
%As stated in Section \ref{sec:limitation_of_existing_works}, there are existing works in data prototype discovery applicable to our problem, and we also incorporate them into the framework of FUNU. We have identified three alternative methods: clustering, confidence, and curvature. 

These existing solutions share a common three-step process. Since they only differ in the first step, we will elaborate on this step in greater detail.

\textbf{Step 1.} Calculate a score $s(x)$ for each sample $x$. The score reflects whether a sample has many similar neighbors in the entire dataset, consistent with the indications of other data prototype discovery methods introduced in Section \ref{sec:limitation_of_existing_works}. In our design, samples with more similar neighbors tend to score lower. The ways to calculate scores for different methods are as follows.

\begin{itemize}
    \item Clustering. Inspired by \cite{carlini2019distribution, Campello2015HierarchicalDE}, we employ a combination of dimensionality reduction and clustering techniques. We apply t-SNE\cite{van2008visualizing} on the pixel space (for dataset MNIST in our experiment) and ResNet-generated feature space (for datasets CIFAR-10 and CIFAR-100) to project the datasets into two dimensions and cluster with HDBSCAN. $s(x)$ for each sample $x$ is its according outlier score~\cite{campello2015hierarchical} in the clustering process.
    \item Confidence\cite{carlini2019distribution}. Model confidence is the output of the final fully connected layer, indicating the probability of the sample belonging to each class. We use softmax to normalize the model output. To adjust the direction of the score, we assign $1-softmax(c(x))$ as the confidence score of $x$, where $c(x)$ is sample $x$'s belonging class and $softmax(i)$ is the model output after softmax on class $i$. 
    \item Curvature\cite{ravikumar2024unveiling, gargmemorization}. The curvature of the network loss around a data point indicates the model's memorization of it. Less rare samples tend to have low curvature. In the original paper~\cite{gargmemorization}, the authors averaged curvatures over many epochs to calculate the final score. However, curvature calculation is timing-consuming (in our experiment, it takes more than one hundred seconds to calculate curvature for one epoch). To maintain competitiveness with other methods, we calculate the curvature only at the second epoch as our $s(x)$. We choose curvature at this epoch because at this stage, the model does not learn too much about the dataset and thus the curvature could reflect how the model reacts to a sample more accurately. Otherwise, if the model were well-trained, it would fit most samples, resulting in uniformly low curvature and it is hard to see the difference. 
\end{itemize}

\textbf{Step 2.} Rank the scores $s(x)$ in ascending order. A lower score indicates the sample has more similar neighbors or is more typical within the entire dataset. 

\textbf{Step 3.} Select $D_u^+ = \{x | s(x) \le \theta \ and \  x \in D_u\}$. As the parameter $\theta$ requires manual selection, it could lead to extensive testing for different parameter choices. In Section \ref{sec:evaluation_on_FUNU-ours}, we select parameters based on the data distribution and show that the results are sensitive to the choice of parameters.

%For these methods, they all follow the same paradigm to find $D_u^-$. In detail, when we apply these methods, firstly, we would calculate a score for each sample. The score calculation methods are specified as follows. 

==> preliminaries_v0_1015.tex <==
In this section, we formulate the concept ``unnecessary unlearning'', and then introduce the problem we aim to address in this paper. We also elaborate on the implementation details and limitations of existing solutions which are applicable to our problem.
%We aim to accelerate the unlearning process by avoiding unnecessary unlearning. Specifically, we reduce data removal requests by ignoring samples that have minimal impact on the retrained model. 

\subsection{Problem setting}
\label{sec:problem_formulation}

To introduce our problem, we first define unnecessary unlearning. Assume $A$ is the training process, and $A(D)$ denotes training a model on dataset $D$. In the context of machine unlearning, we start with an original model $M_o$ trained on the complete dataset $D_o$, i.e., $M_o = A(D_o)$. Subsequently, data removal requests $D_u$, also referred to as unlearning dataset, are received. The model trained on remained dataset $D_r = D_o \backslash D_u$ is denoted as $M_r = A(D_r)$. 

To describe the similarity between models, we use readout functions~\cite{golatkar2020eternal, golatkar2021mixed, golatkar2020forgetting}. Readout functions $f(M)$ indicate the information that can be extracted given a model $M$. Common readout functions include model output, accuracy on the model prediction, etc. $Dist(\cdot)$ is the distance measurement to quantify the distance between the outputs of readout functions for different models. It can be measured using metrics such as KL-divergence, norm, etc. With these components, the definition of unnecessary unlearning is as follows.

\begin{definition}[Unnecessary Unlearning]
Given the remaining dataset $D_r$, the data removal requests $D_u$, and the training process $A$, the unlearning process over $D_u$ is $\epsilon$-unnecessary unlearning if $$Dist(f(A(D_r)), f(A(D_r \cup D_u))) \le \epsilon$$
\end{definition}

It is important to note that the form of the indicator for unnecessary unlearning, $Dist(f(A(D_r)), f(A(D_r \cup D_u)))$, aligns with the definition of unlearning presented in previous works ~\cite{golatkar2020eternal, golatkar2021mixed, golatkar2020forgetting}. However, these works employ different choices for $Dist(\cdot)$ and the readout functions. The underlying idea of this definition is that, an unlearning process which would not produce a model distinguishable (as measured by $\epsilon$) from the original one, is considered unnecessary unlearning. 

Figure \ref{fig:definition} illustrates the definition of unnecessary unlearning and contains the notations we used throughout this paper. With this definition, we further formulate the problem we aim to address in this paper: Given the remaining dataset $D_r$, an unlearning dataset $D_u$, and the training process $A$, \textbf{how to select $D_u^+ \in D_u$, so that the unlearning over $D_u^+$ would lead to $\epsilon$-unnecessary unlearning?}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.85\linewidth]{figures/definition-crop}
  \caption{Definition of unnecessary unlearning}
  \label{fig:definition}
\end{figure}

$D_u^-$ represents the remaining removal requests, defined as $D_u^- = D_u \backslash D_u^+$. After selecting $D_u^+$ from $D_u$, the unlearning process would continue to be performed on $D_u^-$. However, since $|D_u^-|$ is smaller than $|D_u|$, unlearning $D_u^-$ would consume less time and resources.


\subsection{Existing solutions}
\label{sec:alternative_methods}

To address our problem, works in the data prototype discovery field are highly relevant. The focus of this field is to find typical samples that best represent the whole dataset~\cite{carlini2019distribution}. The discovered prototypes can be regarded as the summary of the dataset. They can also be used to enhance training efficiency as well as explain model behavior~\cite{NEURIPS2018_8a7129b8}. We first review existing works in data prototype discovery, summarize these works and their limitations in efficiency in Table \ref{tab:ExistingPrototype}, and then introduce methods applicable to our problem.

\begin{table}[ht]
\centering
%\vspace{-1.0em}
\caption{Existing data prototype discovery methods and their limitations in efficiency}
\label{tab:ExistingPrototype}
\begin{tabular}{ll}
\toprule
Methods                                      & Limitations in efficiency                                                                                       \\
\midrule
\cite{stock2018convnets}, \cite{Carlini2022ThePO}, adv\cite{carlini2019distribution}                      & Need extra attack                                                                                    \\
\cite{feldman2020does}, \cite{feldman2020neural}, priv,ret,agr\cite{carlini2019distribution} & Need retraining/training                                                                             \\
\cite{li2018deep}, \cite{maini2022characterizing},\cite{NEURIPS2018_8a7129b8}                                & \begin{tabular}[c]{@{}l@{}}Need to modify the model \\ architecture or training process\end{tabular} \\
\cite{kim2016examples}                                       & Need to solve an NP problem                                                                    \\
Existing solutions\cite{ravikumar2024unveiling, gargmemorization,carlini2019distribution}                   & -                                                                                                   \\
\bottomrule
\end{tabular}
\vspace{-1.0em}
\end{table}

\subsubsection{Methods with limitation in efficiency.} As shown in Table \ref{tab:ExistingPrototype}, methods proposed in \cite{stock2018convnets}, \cite{Carlini2022ThePO} and the adv indicator proposed in \cite{carlini2019distribution} require extra Membership Inference Attack (MIA) to decide the typicality of data points. However, MIA needs to train shadow models, which could incur costs comparable to retraining a model. Consequently, the cost of identifying $D_u^+$ may be similar to or even exceed the cost of retraining, thereby contradicting the objective of machine unlearning, which is to achieve a model similar to the retrained model while avoiding the retraining cost.

Methods proposed in \cite{feldman2020does, feldman2020neural}, priv, ret and agr\cite{carlini2019distribution} selects prototypes by testing on models trained without the selected data, which inherently includes a retraining process in their methodology. Such methods also conflict with the objective of machine unlearning.

Methods proposed in \cite{li2018deep}, \cite{maini2022characterizing}, and \cite{NEURIPS2018_8a7129b8} attempt to modify model architecture or alter the training process, which is impractical in machine unlearning, as we assume the model has already completed its training. Lastly, the method in ~\cite{kim2016examples} involves searching over an NP problem, which would lead to high computation costs and thus is inefficient for our problem. 

\subsubsection{Details of existing solutions.} Having screened methods that are not suitable in efficiency, we select \textbf{clustering\cite{carlini2019distribution, Campello2015HierarchicalDE}, confidenc-e\cite{carlini2019distribution} and curvature\cite{ravikumar2024unveiling, gargmemorization}} as existing solutions to adapt to our problem. The implementations of these methods are provided in the following. %in Section \ref{sec:alternative_methods}. 

\input{alternative_methods}

\subsection{Limitations of existing solutions}
\label{sec:limitation_of_existing_works}

In this section, we elaborate on the limitations of existing solutions, which we avoid when developing our method. 

\textbf{Limitation 1.} These methods fail to adapt to different types of unlearning scenarios. For example, they can not automatically adjust in random removal and class removal scenarios. The former is to randomly remove samples regardless of their belonging classes, and the latter is to remove samples belonging to the same class. Both scenarios are common in practical unlearning applications.

Intuitively, in the class removal scenario, as the removed samples belong to the same class, that class would experience significant information loss, which would influence the model largely. Consequently, the proportion of $D_u^+$ should be smaller in a class removal scenario than in random removal. However, with existing solutions, the proportion would not vary in different scenarios.

%However, existing works tend to attribute a similar proportion of $D_u^+$ in both class and random removal, as demonstrated in our experiments. 

There is a more fundamental reason for this phenomenon. As illustrated in Figure \ref{fig:limitation1}, existing solutions select $D_u^+$ by evaluating the contribution of each sample in the entire dataset. Specifically, they tend to pick samples that have many similar neighbors in the whole dataset to be $D_u^+$. In this case, as the relationship between the given sample and the entire dataset is fixed, whether a sample would be classified into $D_u^+$ is also fixed, therefore, the proportion of $D_u^+$ remains stable under different unlearning scenarios. However, though a class of data contains samples that have many neighbors in the whole dataset, these samples are less likely to have similar neighbors in the remaining dataset, as their neighbors are also subject to unlearning. Existing solutions fail to identify this difference and thus would leave out samples supposed to be unlearned.

\begin{figure}[h]
  \centering
  \vspace{-0.5em}
  \includegraphics[width=0.9\linewidth]{figures/limitation_1-crop}
  \caption{Existing solutions and our method in class removal scenario}
  \label{fig:limitation1}
  \vspace{-0.5em}
\end{figure}

%There is a more fundamental reason for this phenomenon, and it is this reason that makes existing works unsuitable to the machine unlearning scenario. Existing methods select $D_u^+$ by evaluating the contribution of each sample in the \textbf{entire} dataset, instead of the relative contribution to the \textbf{remaining} dataset. Specifically, they tend to pick samples that have many similar neighbors in the entire dataset to be $D_u^+$, instead of in the remaining dataset. In this case, as the relationship between the given sample and the entire dataset is fixed, whether a sample would be classified into $D_u^+$ is also fixed, therefore, the proportion of $D_u^+$ remains stable under different unlearning scenarios.

Due to this reason, existing solutions are insufficient for solving our problem. Their mechanism dictates that if the samples they find are removed, the model trained on the left dataset would resemble the original model $M_o$. Whereas in our problem, we hope to find samples that lead to the model resembling the retrained model $M_r$. They evaluate the contribution of each sample in the \textbf{entire} dataset, while we focus on the relative contribution to the \textbf{remaining} dataset. 

%Due to different aims, the inability to general unlearning scenarios of existing works is obvious. Take the class removal scenario as an example, in that scenario, a class of data contains samples that have many neighbors in the whole dataset. However, these samples are less likely to have similar neighbors in the remaining dataset, as their neighbors are also subject to unlearning. Existing works fail to identify this difference and thus would leave out samples supposed to be unlearned.

% This phenomenon has a fundamental underlying reason that distinguishes our method from existing works in data prototype discovery. This could lead to bias, for example, when removing a large proportion of samples in a dataset. If a bunch of samples from one class are to be removed, the model would alter largely by distinction, and thus such samples should not be regarded as $D_u^-$. However, by existing works, those samples are likely to be regarded as prototypes due to distribution and thus be classified as $D_u^-$. This is because such methods decide the necessity of unlearning a point simply by looking at the contribution it has to the overall dataset, instead of the remained dataset. 

\textbf{Limitation 2.} These methods require manual parameter selection. Our experiments show that they are sensitive to parameter choices and parameter selection can be challenging in practice.




